StraGo: Harnessing Strategic Guidance for Prompt Optimization

Prompt engineering is pivotal for harnessing the capabilities of large language models (LLMs) across diverse applications. While existing prompt optimization methods improve prompt effectiveness, they often lead to prompt drifting, where newly generated prompts can adversely impact previously successful cases while addressing failures. Furthermore, these methods tend to rely heavily on LLMs' intrinsic capabilities for prompt optimization tasks. In this paper, we introduce StraGo (Strategic-Guided Optimization), a novel approach designed to mitigate prompt drifting by leveraging insights from both successful and failed cases to identify critical factors for achieving optimization objectives. StraGo employs a how-to-do methodology, integrating in-context learning to formulate specific, actionable strategies that provide detailed, step-by-step guidance for prompt optimization. Extensive experiments conducted across a range of tasks, including reasoning, natural language understanding, domain-specific knowledge, and industrial applications, demonstrate StraGo's superior performance. It establishes a new state-of-the-art in prompt optimization, showcasing its ability to deliver stable and effective prompt improvements.

==> tables/meta_prompts.tex <==

$\bullet$ \emph{\textit{Collect positive experiences.}}
\begin{tcolorbox}
    {
    \small
       As a logician, you are good at breaking down the internal logic of the problem step by step. \\
       \\
    <prompt>\{\{prompt\}\}</prompt> \\
     <examples>\{\{examples\}\}</examples> \\
     \\
    I have provided you with a prompt and several examples that include triples of questions, actual answers, and reference answers. Your task is to summarize the \{\{num\}\} most valuable key points to improve your accuracy in solving this type of task.
    }
    
    % \vspace{-5pt}
\end{tcolorbox}
% \newpage
$\bullet$ \emph{\textit{Collect negative experiences.}}
\begin{tcolorbox}
    {
    \small
       As a logician, you are good at breaking down the internal logic of the problem step by step. \\
       \\
    <prompt>\{\{prompt\}\}</prompt> \\
     <examples>\{\{examples\}\}</examples> \\
     \\
    I have provided you with a prompt and several examples that include triples of questions, wrong answers, and reference answers. Your task is to identify \{\{num\}\} primary reasons why the prompt causes these wrong answers.
    }
    
\end{tcolorbox}
$\bullet$ \emph{\textit{Generate strategy.}}
\begin{tcolorbox}
    {
    \small
       As an expert in prompt engineer, your task is to create a step-by-step strategy guide on how to use specific experience based on provided prompt. \\
       \\
        \# Begin Example \\
        \{some examples include prompt, example, experience and strategy\}\\
        \# End Example \\ 
     \\
    My current prompt is: \\
    <prompt>\{\{prompt\}\}</prompt> \\
    \\
    And Here are some task data:\\
    <examples>\{\{examples\}\}<examples>\\
    \\
    Through comprehensive analysis of the data, I've gained an experience that can improve the prompt:\\
    <experience>\{\{experience\}\}</experience>
    }
\end{tcolorbox}

$\bullet$ \emph{\textit{Score}}
\begin{tcolorbox}
    {
    \small
       As an experienced prompt engineering expert, your task is to evaluate a proposed strategy based on a specific experience. Rate the strategy for its appropriateness, clarity, and effectiveness in addressing the experience. \\
       \\
        \# Experience\\
        <experience>\{\{experience\}\}</experience>\\
        \\
        \# Strategy \\
        <strategy>\{\{strategy\}\}</strategy> \\
        
    \# Rating Criteria \\
    1. Match with Experience(M): The strategy should be directly aimed at mitigating the issue described in the experience. A perfect alignment where the strategy completely addresses the experience issue scores 100 points, whereas a poor match scores lower, depending on how well it addresses the problem. \\
    2. Clarity of Strategy(C): The strategy must be explained clearly and in detail. A strategy that is easy to understand and can be practically implemented by any teacher scores 100 points, while a strategy that is poorly described scores less or 0. \\
    3. Effectiveness in Addressing the Issue(E): Consider how comprehensively the strategy deals with preventing errors and promoting understanding in steps. A strategy that effectively addresses both what should do and what should avoid to minimize errors scores 100 points. A strategy that partially addresses these aspects scores less. \\
    \\
    We asked 5 experts to rate the strategy. Each expert evaluate the strategy independently.\\
    \\
    \# Output Format:
    [\{'M': 78, 'C': 85, 'E': 90\}, \{'M':45,...] \\
    \\
    \# Output
        [\{
    }    
\end{tcolorbox}

$\bullet$ \emph{\textit{Optimize.}}
\begin{tcolorbox}
    {
    \small
       My current instruction is: \\
       <prompt>\{\{prompt\}\}</prompt> \\
       \\
        And Here are some task data: \\
        <examples>\{\{examples\}\}<examples> \\
        \\
        Through comprehensive analysis of the data, I get a experience and corresponding strategy:\\
        \\
        \# Experience \\
        <experience>{{experience}}</experience> \\
        \# Strategy \\
        <strategy>\{\{strategy\}\}</strategy> \\
        \\
        Based on my current prompt, refer to this experience and the strategy, write 1 different improved prompt.
        The improved prompt is:
    }
\end{tcolorbox}

$\bullet$ \emph{\textit{Crossover.}}
\begin{tcolorbox}
    {
    \small
      As an experienced instruction writer, your task is to carefully analyze the provided task cases and instructions in order to generate an improved instruction that will guide an AI system to solve the task more effectively.\\
       \\
       \# Task Cases\\
        The task cases and instructions can be found below: \\
        \{\{examples\}\} \\
        % \\
        \# Instruction 1 \\
        \{\{prompt1\}\} \\
        % \\
        \# Instruction 2 \\
        \{\{prompt2\}\} \\
        \\
        Please use the following step-by-step process:\\
        - Step 1: Review the task cases to understand the key objectives and requirements that the instruction needs to address.\\
        - Step 2: Analyze Instruction 1 and identify its strengths and weaknesses in terms of guiding the AI system to solve the task.\\
- Step 3: Perform the same analysis on Instruction 2.\\
- Step 4: Determine how to best combine the strengths of the two instructions while addressing their individual weaknesses.\\
- Step 5: Write an improved, combined instruction that incorporates the insights from the previous steps. The instruction should provide clear guidance for the AI system to solve the task based on the given task cases.\\
- Step 6: Output the improved instruction surrounded by XML tags as follows:\\
<instruction>\\
Your improved instruction goes here.\\
</instruction>
    }
\end{tcolorbox}


$\bullet$ \emph{\textit{Synonyms.}}
\begin{tcolorbox}
    {
    \small
        \# Instruction-Score\\
        \{\{instruction\_score\}\} \\
        \\
        Mutate the following instruction reference [\# Instruction-Score] and generate a better instruction.\\
        \\
        \{\{instruction\}\}\\
        \\
        New instruction:
    }
\end{tcolorbox}
